(Perhaps) Beyond Human Translation: Harnessing Multi-Agent Collaboration for Translating Ultra-Long Literary Texts

Literary translation remains one of the most challenging frontiers in machine translation due to the complexity of capturing figurative language, cultural nuances, and unique stylistic elements. In this work, we introduce TransAgents, a novel multi-agent framework that simulates the roles and collaborative practices of a human translation company, including a CEO, Senior Editor, Junior Editor, Translator, Localization Specialist, and Proofreader. The translation process is divided into two stages: a preparation stage where the team is assembled and comprehensive translation guidelines are drafted, and an execution stage that involves sequential translation, localization, proofreading, and a final quality check. Furthermore, we propose two innovative evaluation strategies: Monolingual Human Preference (MHP), which evaluates translations based solely on target language quality and cultural appropriateness, and Bilingual LLM Preference (BLP), which leverages large language models like GPT-4} for direct text comparison. Although TransAgents achieves lower d-BLEU scores, due to the limited diversity of references, its translations are significantly better than those of other baselines and are preferred by both human evaluators and LLMs over traditional human references and GPT-4} translations. Our findings highlight the potential of multi-agent collaboration in enhancing translation quality, particularly for longer texts.

==> 3_method.tex <==
\section{\ours: A Multi-Agent Virtual Company for Literary Translation}

% \input{figures/transagents}

% We establish a virtual multi-agent translation company, \ours, featuring a diverse range of employees including a CEO, senior editors, junior editors, translators, localization specialists, and proofreaders. When a human client assigns a book translation task, a team of selected agents from \ours collaborates to translate the book. This paradigm simulates the entire book translation process, where agents with different roles work together to ensure that the translation maintains high quality and consistency throughout. In this section, we describe the company overview of \ours in \autoref{sec:overview}, the core collaboration strategies of \ours in \autoref{sec:collab_strategy}, and the translation workflow in \autoref{sec:workflow}. 

\input{figures/workflow}
\revised{The workflow is \autoref{fig:workflow}}

We establish a virtual multi-agent translation company, \ours, featuring a diverse team including a CEO, senior editors, junior editors, translators, localization specialists, and proofreaders. When a human client assigns a book translation task, a selected team from \ours collaborates to translate the book. This approach simulates the entire translation process, ensuring high quality and consistency through the coordinated efforts of agents with various roles. In this section, we describe the company overview of \ours in \autoref{sec:overview}, the core collaboration strategies of \ours in \autoref{sec:collab_strategy}, and the translation workflow in \autoref{sec:workflow}. 



\subsection{Company Overview}
\label{sec:overview}

To simulate the entire book translation process, \ours involves a diverse range of roles besides the CEO, including senior editors, junior editors, translators, localization specialists, and proofreaders, as shown in \autoref{fig:company}, each with distinct responsibilities: 
\begin{itemize}
    \item \textbf{Senior Editors}: Senior editors are responsible for overseeing the content production process. Their primary duties encompass setting editorial standards, guiding other team members, and making decisions regarding publication schedules and content direction.
    \item \textbf{Junior Editors}: Junior editors work under senior editors, managing day-to-day editorial workflows, editing content, and assisting in content planning, and handling communications with various roles within the team.
    \item \textbf{Translators}: Translators convert written material from one language to another, preserving the original text's tone, style, and context.
    \item \textbf{Localization Specialists}: Localization specialists adapt content for specific regions or markets, translating and adjusting cultural references to resonate with local audiences.
    \item \textbf{Proofreaders}: Proofreaders perform final checks for grammar, spelling, punctuation, and other possible errors.
\end{itemize}

\input{figures/profile_example}

\paragraph{Agentization} To enhance the realism and efficacy of our translation process simulation, we use \gptfour to generate 30 diverse virtual agent profiles for each role. As shown in \autoref{fig:profile_example}, these profiles encompass a wide range of attributes beyond language skills, including gender, nationality, rate per word, education, experience, and more. This detailed approach enriches the simulation's authenticity and reflects the complexity and diversity of real-world translation settings, thereby supporting and inspiring future research.

% To enhance the realism and efficacy of our simulation in the translation process, we strategically utilize \gptfour to generate a diverse set of 30 virtual agent profiles for each distinct role. As illustrated in \autoref{fig:profile_example}, these profiles are comprehensively designed to include a wide array of attributes that extend well beyond language skills. Key characteristics such as gender, nationality, rate per word, educational background, years of experience, and areas of specialization are thoughtfully incorporated. This detailed and personalized approach not only enriches the authenticity of the translation process simulation but also mirrors the complexity and diversity found in real-world translation settings. The inclusion of such rich, detailed metadata about the agents not only enhances current simulation strategies but is also designed to support and inspire future research.

\subsection{Agentic Collaboration}
\label{sec:collab_strategy}
In this section, we introduce two collaboration strategies used in this work, including \textit{Addition-by-Subtraction Collaboration} (\autoref{alg:add_by_sub}) and \textit{Trilateral Collaboration} (\autoref{alg:trias}).

\input{algorithms/add_by_subtract}
\paragraph{Addition-by-Subtraction Collaboration}
% In our framework, we propose the \textit{Addition-by-Subtraction Collaboration} between two agents. Unlike the debate-style strategy \citep{DBLP:journals/corr/abs-2305-19118,DBLP:journals/corr/abs-2305-14325,DBLP:journals/corr/abs-2308-07201}, where multiple agents propose their own answers and a third-party agent concludes the discussion, our strategy involves only two agents. One acts as an \textit{Addition agent}, responsible for extracting as much relevant information as possible, while the other agent serves as a \textit{Subtraction agent}, tasked with reviewing the extracted information, eliminating redundant details, and providing feedback to the Addition agent. We present the details of our collaboration strategy in \autoref{alg:add_by_sub}. The Addition agent $\rmA$ first generates the initial response, aiming to include as much informative content as possible. Subsequently, the Subtraction agent $\rmS$ reviews the response and removes any redundant information. The conversation iterates until no further revisions are needed for the response.

In our framework, we introduce the \textit{Addition-by-Subtraction Collaboration} between two agents. Unlike the debate-style strategy, which involves multiple agents proposing answers and a third-party agent concluding, our method uses only two agents. One is the \textit{Addition agent}, who extracts extracting as much relevant information as possible, and the other is the \textit{Subtraction agent}, who reviews and eliminates redundant details, providing feedback to the Addition agent.  We present the details of our collaboration strategy in \autoref{alg:add_by_sub}. The Addition agent $\rmA$ generates an initial response with comprehensive content. The Subtraction agent $\rmS$ then reviews this response, removes redundancies, and the agents iterate this process until no further revisions are necessary. 
\revised{Note that the maximum number of iterations used in \autoref{alg:add_by_sub} is 2.}

\paragraph{Trilateral Collaboration}
% We divide the collaboration into three branches in \ours, referring to as \textit{Trilateral Collaboration}:
% \begin{itemize}
%     \item \textbf{Action}: The power to follow the instruction and implement the required actions.
%     \item \textbf{Critique}: The power to review the generated response and provide constructive feedback to the Action branch.
%     \item \textbf{Judgment}: The power to make the final decision on whether the response is satisfactory or requires further revision.
% \end{itemize}
% We assign one agent for each branch and present the details of the collaboration among these agents in \autoref{alg:trias}. The \textit{Action agent} $\rmP$ generates a response $\rmR$ given the context $\rmC$ and instruction $\rmI$. The \textit{Critique agent} $\rmQ$ then writes critiques $\rmF$ against the response $\rmR$. The Action agent $\rmP$ has the option to either accept the critiques and update the response or maintain the original response. At the end of the iteration, the \textit{Judgment agent} $\rmJ$ evaluates the response $\rmR$ to determine if the discussion can be concluded or if further deliberation is required.

We divide the collaboration in \ours into three branches, referred to as \textit{Trilateral Collaboration}:
\begin{itemize}
    \item \textbf{Action}: Executes instructions and implements required actions.
    \item \textbf{Critique}: Reviews the response and provides constructive feedback to the Action branch.
    \item \textbf{Judgment}: Makes the final decision on whether the response is satisfactory or needs further revision.
\end{itemize}
Each branch is managed by a dedicated agent as detailed in \autoref{alg:trias}. The \textit{Action agent} $\rmP$ generates a response $\rmR$ based on the context $\rmC$ and instruction $\rmI$. The \textit{Critique agent} $\rmQ$ then critiques the response $\rmR$. The \textit{Action agent} $\rmP$ can either accept the critiques and update the response or maintain the original response. Finally, the \textit{Judgment agent} $\rmJ$ evaluates the response $\rmR$ to decide if the discussion can be concluded, \textit{without requiring the conversation history}, due to the agents' limited capability of processing long-range context. 
\revised{Note that the maximum number of iterations used in \autoref{alg:trias} is 2.}

% \paragraph{Judgment Agent in \autoref{alg:trias}}
% We introduce the Judgment Agent in \autoref{alg:trias}, which is responsible for evaluating the quality of the response and determining whether further revision is needed, \textit{without requiring the conversation history}. Owing to the nature of web novels, each turn of dialogue is likely to contain a few thousand words. Although recent advances in large language models (LLMs) claim that LLMs are capable of processing extremely lengthy sequences of up to millions of tokens, we still observe that our agents are not able to effectively leverage the information in the context as the conversation expands. Additionally, we observe that the meaning of translations tends to deviate from the original text after several iterations of revision. Therefore, it is critical to have the Judgment agent within the \textit{Trilateral Collaboration} to ensure the overall quality of the response.


\input{algorithms/trias}
\subsection{Translation Workflow}
\label{sec:workflow}

In this section, we introduce the book translation workflow in our company \ours, including two main stages: preparation (\autoref{sec:prep}) and execution (\autoref{sec:exec}). In the preparation stage, translation guidelines are documented, while in the execution stage, the book is translated and polished.

\subsubsection{Preparation}
\label{sec:prep}

\paragraph{Project Member Selection}
% In our company's setup, we create 30 agent profiles for each role, each accompanied by a unique role assignment prompt, as illustrated in \autoref{fig:profile_example}. These prompts are essential for assigning specific roles to the agents before the dialogues begin. Within our framework, the initial step involves the CEO selecting a Senior Editor for the book translation project. This selection process takes into account both the client's requirements and the qualifications of potential Senior Editors. Once the Senior Editor is chosen, they work closely with the CEO to assemble the rest of the project team, carefully considering the skill sets and backgrounds of the candidates. Furthermore, we introduce a \textit{self-reflection} strategy \citep{DBLP:conf/iclr/YaoZYDSN023, shinn2023reflexion, DBLP:journals/corr/abs-2307-07924}. This strategy involves incorporating a ``ghost agent'' whose task is to prompt the CEO to reconsider their decision, as we observe that they sometimes struggle to select a Senior Editor with the desired language skills.

In our company, we create 30 agent profiles for each role, each with a unique role assignment prompt (see \autoref{fig:profile_example}). These prompts help assign specific roles to agents before dialogues begin. Initially, the CEO selects a Senior Editor for the book translation project, considering the client's requirements and the candidates' qualifications. Once chosen, the Senior Editor collaborates with the CEO to form the project team, taking into account the candidates' skills and backgrounds. Additionally, we employ a \textit{self-reflection} strategy \citep{DBLP:conf/iclr/YaoZYDSN023, shinn2023reflexion, DBLP:journals/corr/abs-2307-07924} by using a ``ghost agent'' to prompt the CEO to reconsider their decision, as they sometimes struggle to select a Senior Editor with the necessary language skills.

\input{figures/guideline}

\paragraph{Long-Term Memory Management}
One of the principal challenges in literary translation is to maintain the coherence, cohesion, and consistency throughout the translated text. In this work, we classify memory into two types: : \textit{short-term memory}, which pertains to the context within the current conversation, and \textit{long-term memory}, which relates to the context spanning the entire book. Recent efforts allow LLMs for effectively processing the sequence containing several thousands of tokens \citep{DBLP:journals/corr/abs-2309-16039,DBLP:journals/corr/abs-2312-00752,DBLP:journals/corr/abs-2404-07839}, but they remain inadequate for handling the broader context required for entire books \citep{DBLP:journals/corr/abs-2406-16264}. Addressing this limitation, we employ multi-agent collaboration to develop a comprehensive set of translation guidelines, guiding all the agents involved in the translation process. In \ours, there are five components in the translation guidelines: the glossary, the book summary, the tone, the style, and the target audience. We design different strategies to process them:
\begin{itemize}
    \item \textbf{Glossary and Book Summary}: The glossary of the book compiles essential terms from the source language and provides their corresponding translations in the target language, while the book summary provide a comprehensive overview of the whole book. Both components are facilitated by the collaboration between the Junior Editor (Addition Agent $\rmA$) and the Senior Editor (Subtraction Agent $\rmS$), employing the \textit{Addition-by-Subtraction Collaboration} as depicted in \autoref{alg:add_by_sub}. In this process, the Junior Editor aims to retain as much detail as possible, while the Senior Editor focuses on removing redundant information.
    
    \item \textbf{Tone, Style, and Target Audience}: The translation of a book is more than just a word-for-word conversion; it's a delicate process of adapting tone, style, and content to resonate with the target audience while staying true to the original text's essence. In \ours, the Senior Editor defines the tone, the style, and the target audience of the translated book based on a randomly selected chapter.
    
\end{itemize}
Overall, the glossary, book summary, tone, style, and target audience together form the comprehensive translation guidelines. These guidelines are prefixed as an essential part of the prompts for all roles involved in the translation process. We present an example prompt used by the Translator in \autoref{fig:guideline}.


\subsubsection{Execution}
\label{sec:exec}

% In the execution phase, the process is divided into four distinct sub-stages: translation, cultural adaptation, proofreading, and final review. During the first three sub-stages, our approach utilizes the collaborative strategy as illustrated in \autoref{alg:trias}. Within this framework, the roles of Action agents $\rmP$ are assigned to the Translator, the Localization Specialist, and the Proofreader, in that order. Meanwhile, the responsibilities of the Critique agent $\rmQ$ and the Judgment agent $\rmJ$ are fulfilled by the Junior Editor and the Senior Editor, respectively. Finally, the Senior Editor performs the final checks before publication.

In the execution phase, the process is divided into four sub-stages: translation, cultural adaptation, proofreading, and final review. The first three sub-stages employ a collaborative strategy as detailed in \autoref{alg:trias}. Here, the Translator, Localization Specialist, and Proofreader act as Action agents $\rmP$. The Junior Editor serves as the Critique agent $\rmQ$, and the Senior Editor functions as the Judgment agent $\rmJ$. The Senior Editor also conducts the final checks before publication.

\paragraph{Translation, Localization, and Proofreading}
% The translation stage involves three key roles: the Translator, the Junior Editor, and the Senior Editor. These roles collaborate to translate the book from the source language to the target language on a chapter-by-chapter basis. The translation process begins with the Translator (the Action agent $\rmP$) initially translating the chapter content from the source language to the target language. Next, the Junior Editor (the Critique agent $\rmQ$) undertakes a thorough review of the translation, ensuring it adheres to the guidelines while also identifying any potential errors or areas for improvement. Lastly, the Senior Editor (the Judgment agent $\rmJ$) evaluates the translation and determines if further revision is needed. Following the translation, the cultural adaptation process begins. The Localization Specialist tailors the translated content to fit the cultural context of the target audience, ensuring that it resonates well and maintains the intended meaning. Next, the Proofreader perform the checks for language errors. Throughout the cultural adaptation and proofreading stages, both the Junior Editor and the Senior Editor continue to offer critiques and evaluations to refine the content further.


The translation stage involves three key roles: the Translator, the Junior Editor, and the Senior Editor, who collaborate to translate the book from the source language to the target language on a chapter-by-chapter basis. The process starts with the Translator (Action agent $\rmP$) translating the chapter content. The Junior Editor (Critique agent $\rmQ$) then reviews the translation, ensuring it adheres to guidelines and identifying any potential errors or areas for improvement. Lastly, the Senior Editor (Judgment agent $\rmJ$) evaluates the translation and decides if further revision is needed. Following translation, the cultural adaptation process begins. The Localization Specialist adapts the content to fit the cultural context of the target audience, ensuring it resonates well and maintains the intended meaning. Next, the Proofreader then checks for language errors. Throughout cultural adaptation and proofreading, both the Junior Editor and the Senior Editor continue to critique and evaluate the content for further refinement.

\paragraph{Final Review}
% The final review is the concluding step in the editorial process. At this point, the Senior Editor evaluates the translation quality of each chapter and also examines how pairs of adjacent chapters flow into each other. The Senior Editor not only verifies that each chapter is internally coherent and meets quality standards on its own but also ensures that the transitions between chapters are smooth, thereby maintaining narrative consistency.

The final review is the concluding step in the editorial process. Here, the Senior Editor evaluates the translation quality and checks the flow between adjacent chapters. The review ensures each chapter is coherent and meets quality standards while maintaining smooth transitions for narrative consistency.




% \subsection{Project Initiation}
% \label{sec:init}

% In the project initiation phase, \ours is tasked with translating a book by a human client. This phase involves two crucial roles: the CEO and the Senior Editor. They collaborate together to choose the members of the project team. 


% \paragraph{Project Member Selection}
% System prompts or messages are commonly used to assign roles to individual agents during the role-playing process. As part of our company setup, we create 30 agent profiles, each accompanied by its unique role assignment prompts, as illustrated in \autoref{fig:profile_example}. These prompts play a crucial role in assigning specific roles to the agents before the dialogues start. In our framework, the initial step involves the CEO selecting a Senior Editor for the book translation project. This selection takes into account both the client's requirements and the qualifications of potential Senior Editors. Once the Senior Editor is chosen, they collaborate closely with the CEO to assemble the rest of the project team, carefully considering the skill sets and backgrounds of the candidates. Following the approach described by \citet{DBLP:journals/corr/abs-2307-07924}, we implement the use of \textit{inception prompting} \citep{DBLP:journals/corr/abs-2303-17760} to achieve role specialization. These prompts contain essential information, including designated tasks and roles, translation guidelines, termination criteria, various constraints, and so on.

% \input{figures/multi_agent_discussion}
% \paragraph{Multi-Agent Discussion}
% \citet{DBLP:journals/corr/abs-2303-17071} propose a multi-agent approach aimed at enhancing the effectiveness of Large Language Models (LLMs) in tackling complex Natural Language Processing (NLP) tasks by facilitating a dialogue between two distinct agents. In our framework, the CEO and the Senior Editor engage in discussions about potential candidates for various roles, as depicted in \autoref{fig:multi_agent_discussion}. The Senior Editor provides candidate recommendations to the CEO, taking into account both the client's requirements and the candidate's qualifications. Subsequently, the CEO is tasked with making the final decision regarding the appointment. The conversation concludes if the CEO deems the recommended candidate suitable for the project. If the CEO does not find the recommended candidate suitable, the Senior Editor is required to propose an alternative candidate.


% \paragraph{Self-Reflection}
% We observe instances where the CEO occasionally fails to select the most suitable Senior Editor with the required language proficiency. For example, when a client requests a book translation from Chinese to English, and the Senior Editor chosen by the CEO may not possess adequate proficiency in either Chinese or English. This erroneous choice can lead to the entire translation process's failure due to the selected Senior Editor lacking the essential language skills necessary for the task. To address this issue, we introduce a \textit{self-reflection} strategy \citep{DBLP:conf/iclr/YaoZYDSN023, shinn2023reflexion, DBLP:journals/corr/abs-2307-07924}. This strategy involves the incorporation of a ``ghost agent'' whose task is to prompt the CEO to reconsider their decision. It effectively enhances the CEO's decision-making performance.


% \subsection{Translation Guideline Documentation}
% \label{sec:guideline}
% This phase requires the collaboration between two roles: the Senior Editor and the Junior Editor. Together, they work on translation guidelines used for book translation project, including documenting the glossary and its translation, establishing the tone and style of the translated book, understanding the target audience, and summarizing the book's content. 

% \paragraph{Addition-by-Subtraction Discussion}
% In our framework, we propose the \textit{Addition-by-Subtraction Discussion} between the Senior Editor and the Junior Editor. Unlike the debate-style strategy \citep{DBLP:journals/corr/abs-2305-19118,DBLP:journals/corr/abs-2305-14325,DBLP:journals/corr/abs-2308-07201}, where multiple agents propose their own answers and a third-party agent concludes the discussion, our \textit{Addition-by-Subtraction} strategy involves only two agents. One agent acts as a \textit{worker}, responsible for extracting as much information as possible, while the other agent serves as the \textit{controller}, tasked with reviewing the extracted information, eliminating unnecessary details, and concluding the conversation.

% \paragraph{Glossary}
% The primary purpose of a glossary in book translation is to compile essential terms from the source language and provide their corresponding translations in the target language. This is crucial for maintaining consistency and accuracy in the usage of these terms throughout the book, especially since some terms may have multiple acceptable translations.  This process allows us to meticulously identify key terms chapter by chapter and compile them into the glossary.  In our framework, we leverage the \textit{Addition-by-Subtraction} strategy to obtain the key terms in the source language. More specifically, for each chapter, the Junior Editor initially makes an exhaustive attempt to identify all potential key terms. Subsequently, the Senior Editor reviews the identified key terms and removes any generic ones. The conversation continues until the Senior Editor believes that all the key terms for the current chapter are identified. When identifying key terms for a new chapter, they also take into account the existing key terms to prevent duplicates in the glossary. To translate these key terms, we adopt the \textit{Multi-Agent Debate} strategy proposed by \citet{DBLP:journals/corr/abs-2305-19118}. In this approach, the Senior Editor engages in a debate with the Junior Editor to determine the most suitable translations for the key terms based on the content of the chapter. However, in our framework, it is the Senior Editor's responsibility to assess the translation quality and conclude the conversation, eliminating the need for a third-party agent.

% \paragraph{Summarization}
% Book summarization plays a vital role in the translation process, providing translators with a concise yet thorough grasp of the book's content, themes, and style. This preliminary comprehension is indispensable as they embark on the intricate task of translation. Despite the ability of modern Large Language Models (LLMs) to handle texts comprising hundreds of thousands of tokens, their context window may still fall short for certain book genres. For instance, while most novels typically consist of 10 to 30 chapters, Chinese web novels can span across hundreds or even thousands of chapters. Moreover, recent LLMs may struggle to capture the nuances present in these exceptionally lengthy texts. In our framework, we also employ the \textit{Addition-by-Subtraction} strategy to generate chapter summaries. Initially, the Junior Editor drafts a detailed summary, and then the Senior Editor reviews the summary and removes unnecessary details. After gathering all the chapter summaries, the Senior Editor and the Junior Editor engage in another round of \textit{Addition-by-Subtraction Discussion} to create the book summary.

% \paragraph{Tone, Style, and Target Audience}
% The translation of a book is more than just a word-for-word conversion; it's a delicate process of adapting tone, style, and content to resonate with the target audience while staying true to the original text's essence. This ensures that the translated work faithfully represents the author's vision and provides a comparable reading experience to audiences in different languages. In our framework, the Senior Editor defines the tone, the style, and the target audience of the translated book based on a randomly selected chapter.


% Overall, the glossary, book summary, tone, style, and target audience collectively constitute the comprehensive translation guidelines. \textbf{These guidelines serve as essential part of prompts for all roles involved in the book translation process, ensuring consistency and coherence throughout the entire work.}

% \subsection{Translation}
% \label{sec:translation}

% The translation stage involves three key roles: the Translator, the Junior Editor, and the Senior Editor, who collaborate to translate the book from the source language to the target language on a chapter-by-chapter basis. The translation process begins with the Translator initially translating the chapter content from the source language to the target language. Following this, the Junior Editor undertakes a thorough review of the translation, ensuring it adheres to the guidelines while also identifying any potential errors or areas for improvement. Once the Junior Editor deems the translation to be of high quality, they conclude their work with the Translator and transfer the translation to the Senior Editor for further verification. The Senior Editor follows a similar verification process as the Junior Editor. If, however, the translation falls short of the required quality standards, the Senior Editor rejects the translation and restarts the translation process for the chapter. This additional verification step is necessary, as we often observe ``laziness'' instances where the Translator refuses to follow the suggestions made by the Junior Editor, resulting in inaccuracies in the translation.\footnote{Similar observation is reported at \url{https://community.openai.com/t/why-i-think-gpt-is-now-lazy/534332}.}

% \subsection{Revision}
% \label{sec:revision}

% The revision stage involves four critical roles: the Localization Specialist, the Proofreader, the Junior Editor, and the Senior Editor. Initially, the Localization Specialist, often in collaboration with the Junior Editor, adapt the translation to align with the target culture. Subsequently, the Proofreader takes over to identify and rectify any errors in the translation. Finally, the Senior Editor performs a comprehensive review of the translation, serving as the last step to guarantee its high quality before publication.

% \paragraph{Cultural Adaptation and Proofreading}
% Cultural adaptation is essential in book translation to bridge the gap between different cultures, allowing literature to transcend linguistic boundaries while preserving its original essence and intent. In our framework, working on a chapter-by-chapter basis, the Localization Specialist initially adapts the translation to the target culture, and then, the Junior Editor reviews the culturally adapted translation. The review step is of vital importance, as we observe that the adaptation is likely to omit some details from the translation, leading to omission and undertranslation issues.

% \paragraph{Consistency Revision}
% Before the book is published, the senior editor conducts a thorough review to ensure that the translation meets the publication standards in terms of quality, accuracy, and style. The senior editor meticulously examines each chapter, assessing its quality. If the senior editor deems the translation to be of high quality, it is approved. However, if any concerns arise regarding the quality, the translation is rejected and sent back to the translation stage (\autoref{sec:translation}).

==> 5_standard_eval.tex <==
\section{Standard Evaluation}
\label{sec:standard_eval}
\input{tables/main_auto}

We present the automatic evaluation results in \autoref{tab:main_auto}. Interestingly, our approach performs poorly in terms of the \dbleu metric, achieving the lowest scores among the compared methods. However, it is important to consider that \dbleu has limitations and may not fully capture the quality and coherence of the generated text. As pointed out by \citet{freitag-etal-2020-bleu}, typical references used for calculating \dbleu scores often exhibit poor diversity and tend to concentrate around translationese language. This suggests that a low \dbleu score does not necessarily imply poor performance of our approach.


Our results align with the findings from \citet{thai-etal-2022-exploring}, who argue that automatic metrics cannot accurately reflect human preference in the context of literary translation. Furthermore, while automatic metrics are typically highly correlated with human judgments based on the Multidimensional Quality Metrics (MQM) framework \citep{burchardt-2013-multidimensional}, this framework may not be suitable for assessing translation quality in the context of literary translation.\footnote{In our preliminary study, we conduct small-scale MQM-based human evaluation and also observe that our approach, \ours, receives a low MQM score.} The unique characteristics and creative aspects of literary texts require a more nuanced evaluation approach that goes beyond the scope of standard automatic metrics and MQM-based human assessments.



==> 6_pref_eval.tex <==
\section{Preference Evaluation}
\label{sec:prefer}

It is crucial to acknowledge that a literary text does not possess a single, universal translation. Conventional translation evaluation methodologies, which typically rely on direct comparisons to a standard reference translation, fail to accommodate the multifaceted and subjective nature of literary texts. Following \citet{thai-etal-2022-exploring}, we engage both human evaluators and  large language models (LLMs) to assess translations based on their preferences. In this section, we describe our methods for preference evaluation in \autoref{sec:prefer_method} and present our results in \autoref{sec:prefer_results}.

\subsection{Evaluation Methods}
\label{sec:prefer_method}

In this section, we propose two preference evaluation methods, \textit{monolingual human preference} (MHP, \autoref{sec:mhp}) and \textit{bilingual LLM preference} (BLP, \autoref{sec:blp}). For both methods, we use the winning rate (\%), which is the percentage of instances where a model's generated chapter is preferred by either the human evaluators (in MHP) or the LLM (in BLP), to measure the model performance.


% However, if the preferred translation system receives the same number of votes as the ``No Preference'' option, we record the preferred translation system as the final preference.

\subsubsection{Bilingual LLM Preference}
\label{sec:blp}
\input{figures/gpt4eval_prompt}
The nature of literary texts, with their inherent complexities, artistic expression, and cultural nuances, makes it virtually impossible to produce a single, universally correct translation. As a result, multiple translations of the same literary text can coexist, each offering a unique perspective and interpretation. Recent works demonstrate that the reference translations are likely to be of low quality \citep{freitag-etal-2023-results, DBLP:journals/corr/abs-2401-08417}. \citet{kocmi-federmann-2023-gemba} demonstrate that \model{gpt-4} is capable of accurately estimating translation quality without the need for human reference translations. Their proposed \model{GEMBA-MQM} metric achieves state-of-the-art performance in WMT 2023 Metric Shared task \citep{freitag-etal-2023-results}.

Motivated by \citet{kocmi-federmann-2023-gemba}, we evaluate the translation segment pairs using \model{gpt-4-0125-preview} without providing the reference translations. Recent research demonstrates that even state-of-the-art LLMs may struggle to process extremely long sequences \citep{DBLP:journals/corr/abs-2308-14508, DBLP:journals/corr/abs-2403-11802, li2024long}. Therefore, we require \model{gpt-4-0125-preview} to determine which translation segment is better as described in \autoref{sec:mhp}, using the prompt shown in \autoref{fig:gpt4eval_prompt}, instead of directly comparing the quality of two entire chapters. We employ a different variant of \model{gpt-4} for evaluation to avoid the potential bias. Given concerns about positional bias in LLM evaluation raised by recent studies \citep{DBLP:journals/corr/abs-2307-03025, DBLP:conf/nips/ZhengC00WZL0LXZ23, dubois2024length}, we evaluate each translation segment pair in both forward and reversed directions.




\subsection{Experiments}
\label{sec:prefer_results}


\paragraph{Setup}
As described in \autoref{sec:datasets}, there are 12 web novels consisting of 240 chapters in our test set. Due to the high cost of human evaluation, we only compare our \ours with the \model{Reference 1} and \model{gpt-4-1106-preview} models. We evaluate the first two chapters of each of the 12 web novels in our test set using both of our preference evaluation methods.


\input{figures/prefer_eval}


\paragraph{Results}
We compare the performance of our \ours with \model{Reference 1} and \model{gpt-4-1106-preview} using monolingual human preference evaluations. The results, presented as winning rates, are shown in \autoref{fig:mhp_eval}. The translations produced by \ours are marginally preferred by human evaluators compared to both \model{Reference 1} and \model{gpt-4-1106-preview}. Additionally, we evaluate the models using bilingual LLM preference, with the results presented in \autoref{fig:blp_eval}. The translations generated by \ours are also more preferred by \model{gpt-4-0125-preview} compared to the other models. Referring to the results in \autoref{tab:lingdiv}, we observe that \model{gpt-4-0125-preview} appears to have a strong preference for diverse and vivid descriptions when evaluating literary translations. We leave the further investigation to the future work.

==> figures/cover_image.tex <==
\begin{figure}[t]
    \centering
    \includegraphics[scale=0.07]{figures/beyond_human.pdf}
    \caption{An illustration of our method. Traditional machine translation (MT) systems often underperform compared to human translators. In this study, we demonstrate that the translations produced by \ours are more preferred by humans than those from conventional MT systems and human translators.}
    \label{fig:cover_image}
\end{figure}

==> figures/transagents.tex <==
\begin{figure}[t]
    \centering
    \includegraphics[scale=0.11]{figures/TransAgents.pdf}
    \caption{\ours, a multi-agent virtual company for literary translation.}
    \label{fig:company}
\end{figure}

==> tables/case_consistency.tex <==
\begin{CJK*}{UTF8}{gbsn}

\begin{table}[t]
% \begin{wraptable}{r}{0.5\textwidth}
\centering
\tiny
\setlength{\tabcolsep}{1pt}
\begin{tabular}{@{}lp{0.33\textwidth}@{}}
\toprule
Original Text              & 第1906章 不思量，自难忘（十二）[OMITTED] 第1907章 不思量，自难忘（十三）[OMITTED]                                                                                   \\ \midrule
\model{Reference 1}        & \textcolor{blue}{Chapter 1906: Unforgettable Memories (12)} [OMITTED] \textcolor{blue}{Chapter 1907: Unforgettable Memories (13)}                                   \\ \midrule
\model{gpt-4-1106-preview} & \textcolor{red}{Chapter 1906: It's Hard to Forget Without Thinking (Twelve)} [OMITTED] \textcolor{red}{Chapter 1907: Without Intention, Unforgettable (Thirteen)} \\ \midrule
\ours                      & \textcolor{blue}{Chapter 1906: Without Intention, Unforgettable (Twelve)} [OMITTED] \textcolor{blue}{Chapter 1907: Without Intention, Unforgettable (Thirteen)}   \\ \bottomrule
\end{tabular}
\caption{
Case study for global consistency.
\textcolor{red}{The text in red} indicates inconsistent translations across different chapters, while \textcolor{blue}{the text in blue} indicates consistent translations.
}
\label{tab:case_consistency}
\end{table}

\end{CJK*}
